Not all Views are Created Equal: Analyzing Viewpoint Instabilities in Vision Foundation Models

In this paper, we analyze the viewpoint stability of foundational models - specifically, their sensitivity to changes in viewpoint- and define instability as significant feature variations resulting from minor changes in viewing angle, leading to generalization gaps in 3D reasoning tasks. We investigate nine foundational models, focusing on their responses to viewpoint changes, including the often-overlooked accidental viewpoints where specific camera orientations obscure an object's true 3D structure. Our methodology enables recognizing and classifying out-of-distribution (OOD), accidental, and stable viewpoints using feature representations alone, without accessing the actual images. Our findings indicate that while foundation models consistently encode accidental viewpoints, they vary in their interpretation of OOD viewpoints due to inherent biases, at times leading to object misclassifications based on geometric resemblance. Through quantitative and qualitative evaluations on three downstream tasks - classification, VQA, and 3D reconstruction - we illustrate the impact of viewpoint instability and underscore the importance of feature robustness across diverse viewing conditions.

==> algorithms/instability_computation_alg.tex <==

\begin{algorithm}[H]
\caption{Instability Computation with Non-Maximum Suppression}
\label{alg:instability_nms}
\begin{algorithmic}[1]
\State \textbf{Input: } featurizer $f$, set of viewpoints $\{v_i\}_{i=1}^{N}$, error threshold $\tau_e$, ball radius $r_e$
\State Compute instability scores $\{\text{err}_f(v_i)\}_{i=1}^{N}$ using Eq.~\ref{err_eq}
\State $\mathcal{U} \gets \emptyset$ 
\For{$i = 1$ to $N$}
    \If{$\text{err}_f(v_i) \geq \tau_e$} 
        \State $is\_local\_maximum \gets \text{True}$
        \For{$v_j \in B(v_i, r_e)$} 
            \If{$\text{err}_f(v_j) > \text{err}_f(v_i)$}
                \State $is\_local\_maximum \gets \text{False}$
                \State \textbf{break}
            \EndIf
        \EndFor
        \If{$is\_local\_maximum$} 
            \State $\mathcal{U} \gets \mathcal{U} \cup \{v_i\}$ 
        \EndIf
    \EndIf
\EndFor
\State \Return $\mathcal{U}$
\end{algorithmic}
\end{algorithm}

==> sec/methods.tex <==
\section{Method: Unstable Viewpoint Identification}
\label{sec:method}
Given an image $I_{v} \in \mathbb{R}^{H \times W}$ of a 3D scene taken at view $v$ (3D position and angle), and an arbitrary model \( f(\cdot): \mathbb{R}^{H\times W} \rightarrow \mathbb{R}^d \) that embeds the image into a $d$-dimensional vector, we aim to measure the model's viewpoint stability at $v$, i.e., how the model's output features $f(I_v)$ respond to a small perturbation in $v$. If such a perturbation causes a large change, we consider these features unstable. In Sec.~\ref{sec:method-label}, we first propose a metric to label viewpoints as stable/unstable, assuming access to a dense set of images taken around a scene. In Sec.~\ref{sec:method-predict}, we then propose methods to classify a view as stable/unstable from a featurizer's output alone, and to separate unstable views into accidental and other sub-types.

\subsection{Unstable Viewpoint Definition}
\label{sec:method-label}
We define two distance functions: $d_v (\cdot, \cdot)$ which measures the distance between two orientations $v_1$ and $v_2$, and $d_f (\cdot, \cdot)$ which measures the distance between two feature vectors $f(v_1)$ and $f(v_2)$. In our experiments, we let $d_v$ encode Euclidean distance based on 3D position and angle, and let $d_f$ encode cosine distance (the most commonly used distance for features of modern foundation models). Further, let $N_v(v_i, r)$ denote the set of all nearest neighbors to $v_i$ such that if $u \in N(v_i, \tau)$, $d_v(v_i, u) \leq r$. We then define the instability score at $v_i$:
\begin{align}
\text{ins}_f(v_i) = \frac{1}{|N_v(v_i, r)|} \sum_{u \in N(v_i, r)} d_f(f(v_i), f(u)).
\label{eq:instability}
\end{align}
We then label \( v_i \) as unstable if $\text{ins}_f(v_i) > \tau$, for some fixed threshold \( \tau \).  
%\begin{align}
%v_i := 
%\begin{cases} 
%    \text{unstable} & \text{if } , \\
%    \text{stable} & \text{otherwise},
%\end{cases}
%\label{eq:unstable}
%\end{align}

Fig.~\ref{fig:instability_plot_examples} illustrates stability scores and unstable viewpoints detected for several examples from the Amazon-Berkeley Objects (ABO) dataset \cite{collins2022abo}. Some objects, such as the side table (Fig.~\ref{fig:instability_plot_examples}-left), have no unstable viewpoints. Others, such as the painting (Fig.~\ref{fig:instability_plot_examples}-center) have accidental viewpoints corresponding to the camera perfectly aligned with the object to conceal its geometry. And yet other objects, such as the cushion (Fig.~\ref{fig:instability_plot_examples}-right) have instabilities which do not appear accidental, but rather are caused by out-of-distribution (OOD) viewpoints or artifacts.  

\subsection{Predicting Viewpoint Instability from Features}
\label{sec:method-predict}

In most real applications, we will not have access to a dense set of neighboring images to a given view. In these cases, we will be unable to apply Eq.~\ref{eq:instability} to determine whether $f(v_i)$ are stable features or not. Hence, we also explore predicting instability from $f(v_i)$ directly. To do so, we propose training a binary classifier to predict these labels from corresponding features, following previous studies that predict semantic attributes from featurizers\gb{~\cite{}}. We train this classifier on a dataset of dense 360-degree scene captures, annotating each view of each scene with stable/unstable labels using Eq.~\ref{eq:instability}.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth, trim={0cm 0cm 0 0}, clip]{figs/pca_abo_3.png} 
    \caption{ \textbf{PCA visualization of stable (blue), unstable-accidental (green), and unstable-OOD (red) viewpoints using CLIP embeddings from ABO dataset} We see that unstable viewpoints cluster in feature space, with accidental viewpoints tightly grouped. Please refer to sample images from the unstable-accidental and unstable-OOD in Fig.~\ref{fig:cluster_sample_combined}. } 
    \label{fig:pca_abo_clip} 
\end{figure}

We further hypothesize that unstable views may be separable into interpretable sub-clusters in feature space. Fig.~\ref{fig:pca_abo_clip} shows a 2D projection of CLIP features on the ABO dataset using Principal Component Analysis (PCA)~\cite{pearson1901liii}, with stable points displayed in blue, and two clusters of unstable points obtained with $k$-means~\cite{macqueen1967some} shown in green and red. Upon visual inspection of samples, we find the green cluster largely corresponds to accidental views, while the red are other out-of-distribution (OOD) views. Interestingly, the green cluster is also ``tighter,'' which agrees intuitively with the idea that these views share similar collapsed 1D/2D structures. We therefore propose to separate accidental from OOD unstable viewpoints in arbitrary feature spaces by fitting $k=2$ clusters on unstable points, and assigning the cluster with highest silhouette score as accidental.

%Given a set of unstable viewpoints densely covering a 3D scene (, we further apply non-maximal-suppression to returning near-duplicate unstable points next to one another in orientation space, we can apply n to sparsify the returned set. 

%certain local regions of the feature space with several unstable points  
%Alternatively, to avoid potentially returning many unstable points next to one another in some parts of the feature sapce, we can apply non-maximal suppression to only return those points with 
%Alternatively, to avoid returning redundant unstable points
%and prevents over-representation of instability in localized areas.
%To ensure that unstable viewpoints are not redundantly detected in dense regions of feature space, we apply a non-maximum suppression (NMS) strategy. Specifically, we define a neighborhood around each feature embedding \( f(v_i) \) as a ball of radius \( r_e \), denoted \( B_e(f(v_i), r_e) \), in feature space. The NMS algorithm identifies the most unstable viewpoint within each neighborhood in feature space and suppresses the others. This process reduces redundancy and prevents over-representation of instability in localized areas.

%The complete procedure for computing instability scores, applying NMS, and labeling viewpoints as either stable or unstable is outlined in Algorithm~\ref{alg:instability_nms}.
%We first present an algorithm in Sec.~\ref{sec:stability} for determining whether a viewpoint is stable given a set of local neighboring views. Third, in Sec.~\ref{sec:unstable-cluster} we present a method to further categorize unstable viewpoints into \emph{\accidental} and \emph{\uncommon} subtypes. Finally, in Sec.~\ref{sec:stability-prediction} we propose a simple method to automatically predict whether a given viewpoint is unstable \textbf{from the model's features alone}. 
